Vehicle-to-grid for car sharing -- A simulation study for 2030

The proliferation of car sharing services in recent years presents a promising avenue for advancing sustainable transportation. Beyond merely reducing car ownership rates, these systems can play a pivotal role in bolstering grid stability through the provision of ancillary services via vehicle-to-grid (V2G) technologies - a facet that has received limited attention in previous research. In this study, we analyze the potential of V2G in car sharing by designing future scenarios for a national-scale service in Switzerland. We propose an agent-based simulation pipeline that considers population changes as well as different business strategies of the car sharing service, and we demonstrate its successful application for simulating scenarios for 2030. To imitate car sharing user behavior, we develop a data-driven mode choice model. Our analysis reveals important differences in the examined scenarios, such as higher vehicle utilization rates for a reduced fleet size as well as in a scenario featuring new car sharing stations. These disparities translate into variations in the power flexibility of the fleet available for ancillary services, ranging from 12 to 50 MW, depending on the scenario and the time of the day. Furthermore, we conduct a case study involving a subset of the car sharing fleet, incorporating real-world electricity pricing data. The case study substantiates the existence of a sweet spot involving monetary gains for both power grid operators and fleet owners. Our findings provide guidelines to decision makers and underscore the pressing need for regulatory enhancements concerning power trading within the realm of car sharing.

==> table.tex <==
\begin{table}[ht]
\begin{tabular}{@{}llll@{}}
\toprule
Name                                & Type      & Dim.                 & Description                                    \\\midrule
$c$                                   & var  & $\mathds{Z}^{T \times n_v}_{\{0,1 \}}$ & ev connected to charger                    \\
$x_{c}$                         & var & $\mathds{Z}^{T \times n_v}_{\{0, 1\}}$              & plug state \\
$x$                                   & var  & $\mathds{R}^{T+1 \times n_{v}}$        & batteries state {[}kWh{]}                        \\
$u_c, u_d$                                    & var  & $\mathds{R}^{T \times n_{v}}$ & charging / discharging power {[}kW{]}        \\
$y$                                   & var  & $\mathds{R}^{T}$          & energy costs {[}£{]}                           \\
$r$                                   & par  & $\mathds{R}^{T}$          & reference profile                           \\
$l$                                   & par  & $\mathds{Z}^{T \times n_{v}}$          & location matrix                           \\
$n_{max, s}$                                   & par  & $\mathds{Z}^{n_{s}}$          & stations' chargers                            \\
$p_{s, max}$                                   & par  & $\mathds{R}^{n_{s}}$          & stations' max power                           \\
$p_{buy}$, $p_{sell}$             & par & $\mathds{R}^T$            & buying and selling prices {[}£/kWh{]}                       \\
$e$                          & par & $\mathds{R}^{T\times n_v}$            & energy constraint matrix {[}kWh{]}   \\
$\Delta e$                          & par & $\mathds{R}^{T\times n_v}$            & $\Delta$ energy at arrival {[}kWh{]}   \\
$\hat{p}$                                & par & $\mathds{R}^T$            & forecasted station power    {[}kW{]}              \\
$\hat{p}_{pv}$                                   & par  & $\mathds{R}^{T}$          & forecasted PV profile                           \\
$x_{start}$                        & par & $\mathds{R}^{n_v}$              & initial battery state {[}kWh{]}                \\

$x_{min}, x_{max}$                         & par & $\mathds{R}^{n_v}$              & capacity limits [kWh] \\
$u_{d, min}, u_{d, max}$                         & par & $\mathds{R}^{n_v \times 2}$              & discharging limits [kW] \\
$u_{c, min}, u_{c, max}$                         & par & $\mathds{R}^{n_v \times 2}$              & charging limits [kW] \\\bottomrule
\\
\end{tabular}
\caption{Variables, parameters and constants of the EV optimization problem.}\label{tab1}
\end{table}
